Kink instability: evolution and energy dissipation in Relativistic Force-Free Non-Rotating Jets

We study the evolution of kink instability in a force-free, non-rotating plasma column of high magnetization. The main dissipation mechanism is identified as reconnection of magnetic field-lines with various intersection angles, driven by the compression of the growing kink lobes. We measure dissipation rates ${\rm d} U_{B\phi}/{{\rm d}t} \approx -0.1 U_{B\phi}/\tau$, where $\tau$ is the linear growth time of the kink instability. This value is consistent with the expansion velocity of the kink mode, which drives the reconnection. The relaxed state is close to a force-free Taylor state. We constraint the energy of that state using considerations from linear stability analysis. Our results are important for understanding magnetic field dissipation in various extreme astrophysical objects, most notably in relativistic jets. We outline the evolution of the kink instability in such jets and derive constrains on the conditions that allow for the kink instability to grow in these systems.

==> macros.tex <==
\newcommand\aj{\rmfamily{AJ}}%
          % Astronomical Journal
\newcommand\araa{\rmfamily{ARA\&A}}%
          % Annual Review of Astron and Astrophys
\newcommand\apj{\rmfamily{ApJ}}%
          % Astrophysical Journal
\newcommand\apjl{\rmfamily{ApJ}}%
          % Astrophysical Journal, Letters
\newcommand\apjs{\rmfamily{ApJS}}%
          % Astrophysical Journal, Supplement
\newcommand\ao{\rmfamily{Appl.~Opt.}}%
          % Applied Optics
\newcommand\apss{\rmfamily{Ap\&SS}}%
          % Astrophysics and Space Science
\newcommand\aap{\rmfamily{A\&A}}%
          % Astronomy and Astrophysics
\newcommand\aapr{\rmfamily{A\&A~Rev.}}%
          % Astronomy and Astrophysics Reviews
\newcommand\aaps{\rmfamily{A\&AS}}%
          % Astronomy and Astrophysics, Supplement
\newcommand\azh{\rmfamily{AZh}}%
          % Astronomicheskii Zhurnal
\newcommand\baas{\rmfamily{BAAS}}%
          % Bulletin of the AAS
\newcommand\jrasc{\rmfamily{JRASC}}%
          % Journal of the RAS of Canada
\newcommand\memras{\rmfamily{MmRAS}}%
          % Memoirs of the RAS
\newcommand\mnras{\rmfamily{MNRAS}}%
          % Monthly Notices of the RAS
\newcommand\pra{\rmfamily{Phys.~Rev.~A}}%
          % Physical Review A: General Physics
\newcommand\prb{\rmfamily{Phys.~Rev.~B}}%
          % Physical Review B: Solid State
\newcommand\prc{\rmfamily{Phys.~Rev.~C}}%
          % Physical Review C
\newcommand\prd{\rmfamily{Phys.~Rev.~D}}%
          % Physical Review D
\newcommand\pre{\rmfamily{Phys.~Rev.~E}}%
          % Physical Review E
\newcommand\prl{\rmfamily{Phys.~Rev.~Lett.}}%
          % Physical Review Letters
\newcommand\pasp{\rmfamily{PASP}}%
          % Publications of the ASP
\newcommand\pasj{\rmfamily{PASJ}}%
          % Publications of the ASJ
\newcommand\pasa{\rmfamily{PASA}}%
          % Publications of the Astronomical Society of Australia
\newcommand\qjras{\rmfamily{QJRAS}}%
          % Quarterly Journal of the RAS
\newcommand\skytel{\rmfamily{S\&T}}%
          % Sky and Telescope
\newcommand\solphys{\rmfamily{Sol.~Phys.}}%
          % Solar Physics
\newcommand\sovast{\rmfamily{Soviet~Ast.}}%
          % Soviet Astronomy
\newcommand\ssr{\rmfamily{Space~Sci.~Rev.}}%
          % Space Science Reviews
\newcommand\zap{\rmfamily{ZAp}}%
          % Zeitschrift fuer Astrophysik
\newcommand\na{\rmfamily{New Ast.}}%
\newcommand\nat{\rmfamily{Nature}}%
          % Nature
\newcommand\iaucirc{\rmfamily{IAU~Circ.}}%
          % IAU Cirulars
\newcommand\aplett{\rmfamily{Astrophys.~Lett.}}%
          % Astrophysics Letters
\newcommand\apspr{\rmfamily{Astrophys.~Space~Phys.~Res.}}%
          % Astrophysics Space Physics Research
\newcommand\bain{\rmfamily{Bull.~Astron.~Inst.~Netherlands}}%
          % Bulletin Astronomical Institute of the Netherlands
\newcommand\fcp{\rmfamily{Fund.~Cosmic~Phys.}}%
          % Fundamental Cosmic Physics
\newcommand\gca{\rmfamily{Geochim.~Cosmochim.~Acta}}%
          % Geochimica Cosmochimica Acta
\newcommand\grl{\rmfamily{Geophys.~Res.~Lett.}}%
          % Geophysics Research Letters
\newcommand\jcp{\rmfamily{J.~Chem.~Phys.}}%
          % Journal of Chemical Physics
\newcommand\jgr{\rmfamily{J.~Geophys.~Res.}}%
          % Journal of Geophysics Research
\newcommand\jqsrt{\rmfamily{J.~Quant.~Spec.~Radiat.~Transf.}}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\newcommand\memsai{\rmfamily{Mem.~Soc.~Astron.~Italiana}}%
          % Mem. Societa Astronomica Italiana
\newcommand\nphysa{\rmfamily{Nucl.~Phys.~A}}%
          % Nuclear Physics A
\newcommand\physrep{\rmfamily{Phys.~Rep.}}%
          % Physics Reports
\newcommand\physscr{\rmfamily{Phys.~Scr}}%
          % Physica Scripta
\newcommand\planss{\rmfamily{Planet.~Space~Sci.}}%
          % Planetary Space Science
\newcommand\procspie{\rmfamily{Proc.~SPIE}}%
          % Proceedings of the SPIE
          
